Learning context-aware adaptive solvers to accelerate quadratic programming

Convex quadratic programming (QP) is an important sub-field of mathematical optimization. The alternating direction method of multipliers (ADMM) is a successful method to solve QP. Even though ADMM shows promising results in solving various types of QP, its convergence speed is known to be highly dependent on the step-size parameter $\rho$. Due to the absence of a general rule for setting $\rho$, it is often tuned manually or heuristically. In this paper, we propose CA-ADMM (Context-aware Adaptive ADMM)) which learns to adaptively adjust $\rho$ to accelerate ADMM. CA-ADMM extracts the spatio-temporal context, which captures the dependency of the primal and dual variables of QP and their temporal evolution during the ADMM iterations. CA-ADMM chooses $\rho$ based on the extracted context. Through extensive numerical experiments, we validated that CA-ADMM effectively generalizes to unseen QP problems with different sizes and classes (i.e., having different QP parameter structures). Furthermore, we verified that CA-ADMM could dynamically adjust $\rho$ considering the stage of the optimization process to accelerate the convergence speed further.

==> sections/01_intro.tex <==
%Intro-paragraph1
The importance of the quadratic program (QP) becomes more significant with various usage, particularly in large-scale problems, such as portfolio optimization, machine learning, and model predictive control. QP’s various usage and challenging real-world constraints have led to the development of methods to solve QP more effectively. Among them, OSQP (Operator Splitting Quadratic Program), based on the Alternating Direction Method of Multipliers (ADMM), has been widely used due to its advantages, such as performing well in large-size problems and providing a fast convergence rate.

ADMM is advantageous for solving QP because it has satisfactory accuracy with cheap computation and simplicity to execute \citep{OSQP}. In the ADMM algorithm, step-size $\rho$ plays a vital role in determining the convergence speed and accuracy. Researchers have proposed various approaches to adaptively determine the $\rho$ parameter to improve the convergence speed. Typically, setting $\rho$ is classified in two ways; (1) adjust the $\rho$ value according to the primal and dual residual’s ratio. (2) calculate $\rho$ through the QP parameter. The OSQP solver, based on ADMM, adjusts $\rho$ by using the square root of the ratio between normalized residuals with their tolerances (i.e., it belongs to (1)).

Recently, reinforcement learning has been used to derive an optimum policy to select the $\rho$ parameters given the iteration status of the solver. Although the effect of the proposed learning-based parameter selection was effective, the performance improvement was limited because the model’s Markov Decision Process (MDP) is not enough to reflect the structural characteristics of the QP and ADMM iterations, and the relationship between QP and ADMM parameters. Also, the model less considered dynamic changes in ADMM iterations while finding the accurate solution. Both limitations make capturing the proper problem context challenging, which means that the RLQP's generalization capability to unseen problem size and class is non-trivial.

In this study, we propose CA-ADMM, an efficient adaptive policy for adjusting the $\rho$ parameter in the QSQP solver, to accelerate the convergence speed of the various types of QP problems. CA-ADMM employs Recurrent Graph Neural Network (GRNN) type encoder to extract (1) the spatial relationships among the optimization variables and the constraint with our new representation of QP via graph; and (2) the temporal relationships on how the internal states of the optimization variables evolve during the iterations of ADMM algorithms. The extracted latent features that capture the context of a target QP are then used to select the optimum $\rho$ to accelerate the convergence, which has been proven to be effective not only outperforming in the trained domain but also in generalizing well to different problem sizes and different problem class (cross-domain transferability).

In experiments, we verified that CA-ADMM could dynamically adjust the $\rho$ considering the structure of the QP and the stage of the ADMM iterations to accelerate the convergence speed further.
To show our algorithm’s distinction, we trained the model in each problem class that OSQP provides and tested it in each train set.
We also verified that the effective spatial-temporal representation scheme allows CA-ADMM can effectively generalize to unseen QP problems with different problem sizes and the form of objective/constraints (cross-domain transferability). 
To show generalization to unseen problems and scalability to large-scale problems, we trained the model in limited class and size and tested it in extended problem class and size.

The novelties of the proposed method are summarized below:
\begin{itemize}
    \item \textbf{Spatial relationships}: CA-ADMM Suggests the new representation of QP based on a graph, and the HGNN extracts spatial context by considering the structure of QP. \item \textbf{Temporal relationships}: CA-ADMM extract temporal context from history, which can reflect relationships on how the internal states of the optimization variables evolve during the iterations of ADMM.
    \item \textbf{Generalization}: CA-ADMM outperforms existing methods for various unseen problem classes and sizes, even if it is learned only from limited domains and without additional training.
\end{itemize}
% \begin{itemize}
% \item \textbf{Higher Performance}: Performance up compared to existing algorithms with a specific number(after every experiment finish)

% \item \textbf{New representation for QP}: Convert QP state to heterogeneous QP, which can consider the connection: (1) between constraint and variable and (2) between variables.

% \item \textbf{Extract context from history}: The algorithm can extract the meaningful context by improving understanding of the QP environment(problem’s characteristic such as matrix $P, A$, and problem class) through history states and actions(better result than learning in various sets at once)

% \item \textbf{contextual learning at QP in problem class and dimension}: The model can extract context suitable for the QP environment from history even if it is never learned from the problem, large size QP problem of a specific problem class. % 조금더 강조해 쓰고 싶음
% \end{itemize}
% Mathematical optimization is a cornerstone of decision-making problems. Out of various mathematical optimization problems,  convex optimization problems is applied to -- due to its optimality guarantee. --


% \ch{Fast convergence of convex optimization is a significant concern in many domains. \textbf{not yet, write about advantage of fast convergence in many fields}.} Among convex optimization, problems in many domains that we mentioned can be converted to quadratic program (QP) due to providing convexity and simplicity from the matrix’s characteristic. Convex QP is treated as seminal work of Linear Program (LP) \citep{Math_Method_planning}. Various algorithms (e.g., first-order, interior point, etc.) have been proposed and developed over the decades. Also, solvers (e.g., MOSEK, GUROBI, CVXGEN, etc.) that can solve convex QPs are created via the algorithms and used in many domains.
% The interior point method, widely used in QP solvers (e.g., Gurobi, Mosek), has a disadvantage because it is challenging to warm-start and scale with the large size of the problem \cite{OSQP}. Therefore, to solve QP, the Alternative Direction Multiplier Method (ADMM) and an Operator-Splitting QP solver, which is based on ADMM, are used frequently.

% A quadratic program can be represented in matrix form:
% \begin{align}
%     \min_{x} \quad & \frac{1}{2}x^TPx + q^Tx  \label{objective_func} \\
%     \text{subject to} \quad & l \leq Ax \leq u \label{constraints_func}
% \end{align}

% %Intro-paragraph2
% The number of iterations required to converge the OSQP solver is affected by various hyperparameters inside the ADMM algorithm. Among them, the penalty parameter $\rho$ is essential in converging iterations [\cite{Distributed_ADMM},  \cite{ADMM_adaptive}, \cite{Optimal_ADMM}, \cite{OSQP}, \cite{RLQP}]. However, there is no straightforward method to find optimal $\rho$, which directly provides minimum iterations to converge for the primal and dual residual. Therefore, People used heuristic methods to find proper $\rho$  [\cite{Distributed_ADMM}, \cite{ADMM_adaptive}, \cite{Optimal_ADMM}, \cite{OSQP}] by using current information from residuals and QP instances. Also, Reinforcement Learning Quadratic Program (RLQP) is used to find appropriate $\rho$  \cite{RLQP} from MDP configuration from the OSQP system, and it outperformed heuristics. 

% %Intro-paragraph3
% RL methods that solve QP use primal and dual residuals as state, $\rho$ as action, and the number of iterations until converging as a reward. Although the algorithm showed much smaller iterations to converge than the heuristics at OSQP, it still has much potential for development.

% \textbf{Reflect QP instance}
% The QP instances $P$ and $A$ were used to obtain powerful $\rho$ \cite{Optimal_ADMM}. The adopting rule of $\rho$ at \cite{Optimal_ADMM} can provide a convergence rate for the upper bound of residuals. Also, it can be used as a powerful heuristic. In particular, Matrices $P$ and $A$ refer to the relationship between constraint and variable and the relationship between variables. However, previous methods have not reflected this matrix's information due to the assumption of heuristic and computation burden. Therefore we construct a state which can reflect information from the matrices $P$ and $A$ via graph representation to converge with fewer iterations.

% \textbf{observability}
% Previous methods did not consider incomplete observability of its state. In QP, a change in the value of a variable component $x_i$ can influence every constraint that $x_i$ belongs. However, in the existing methods, each constraint takes action with only the information of the constraint. Therefore, each state (constraint) is challenging to ensure observability. Moreover, it means that the QP environment belongs to the Partially observable Markov decision process (POMDP), and it is difficult to maintain the Markov property.
% We cannot ensure Markovian in the MDP setting of existing methods. They used residuals' infinity norm as the state. Depending on the characteristic of the QP instance, the constraint corresponding to the infinity norm may vary at every timestep. Nevertheless, methods only used each single timestep information. [\cite{AI_OR_Control}] stated that using a single timestep state alone may not provide the information required to infer the environment's dynamic system. Also, [\cite{Memory_based_DRL}, \cite{DeepRecurrentQ}, \cite{Memory_based_RNN}] showed that using the history of past observations and actions with Recurrent Neural Network (RNN) is beneficial to solving POMDPs

% \textbf{contextual learning}
% We can't always train $\rho$ in the environment we want. Therefore, algorithms that learn in universal QP can be applied to various problem classes are quite important. Training policy by RL has succeeded in finding $\rho$ that can converge faster than the heuristic rule of the existing OSQP. However, fast convergence can only be guaranteed when learning from all problem classes or when the problem classes of train and test are the same.
% The problem class we need to solve in QP is not always provided. Even if it is a problem that belongs to a typical problem class, a significant problem size is disadvantageous if the problem size is large. [\cite{RLQP}] To create a model that converges faster at unseen dimensions and problem class of QP problems is essential. The model has to enhance its understanding of the QP environment more than the present. At the same time, there is a need for an algorithm that expands the problem to the range of contextual learning so that the model can quickly adapt to unseen QP.

% %intro-paragraph4
% We propose QP solver \textbf{"Contextual-RLQP"} that reduces iterations to converge by providing proper penalty parameter $\rho$ at the OSQP solver for each constraint. The algorithm consists of spatial and temporal parts simultaneously capturing necessary information from both sides. The model used Graph Neural Network (GNN) in the spatial component to capture the relation between variables and constraints. In the temporal part, the model used Recurrent Neural Network (RNN) to extract context information from history. To train the policy for Contextual-RLQP, we define $\mathcal{S}$ as a heterogeneous graph representation form of QP, $\mathcal{A}$ as the internal penalty parameter $\rho$ vector for constraints, and $r$ to minimize iterations until converging.

% %intro-paragraph5 수정 필요
% In experiments, we conduct five experiments in different settings. \\
% First, we trained the model in each problem class and tested it in the trained problem class. The purpose of the experiment is to compare each algorithm and baselines' performance by iterations until they converge. Then, we showed our model is better than existing methods by using the spatial and temporal structures when we fix our problem class. \\
% Second, we trained the model at random QP in OSQP that contained every problem class and tested it at each problem class. In the second experiment, we showed our model could be better at unseen problem classes by capturing informative context from spatial and temporal structures.\\
% Third, we trained our model at problem class 'Random QP' with dimension scaling at the test set. We showed our model could do well regardless of problem size. \\
% Fourth, We did an ablation study to check each component's importance to our algorithm. We showed that each part of our algorithm and the heterogeneous graph are essential.
% Lastly, we will generate action and compare it with heuristic rules to check Whether the heuristic method is reasonable.

% %intro-paragraph6
% The contributions of this paper are:
% \begin{itemize}
% \item \textbf{Higher Performance}: Performance up compared to existing algorithms with a specific number(after every experiment finish)

% \item \textbf{New representation for QP}: Convert QP state to heterogeneous QP, which can consider the connection: (1) between constraint and variable and (2) between variables.

% \item \textbf{Extract context from history}: The algorithm can extract the meaningful context by improving understanding of the QP environment(problem’s characteristic such as matrix $P, A$, and problem class) through history states and actions(better result than learning in various sets at once)

% \item \textbf{contextual learning at QP in problem class and dimension}: The model can extract context suitable for the QP environment from history even if it is never learned from the problem, large size QP problem of a specific problem class. % 조금더 강조해 쓰고 싶음
% \end{itemize}

==> sections/background_subscript.tex <==
\label{section:bacgroud}
\paragraph{Quadratic programming (QP)} A quadratic program (QP) associated with $N$ variables and $M$ constraints is an optimization problem has the form of following:
\begin{equation}
\begin{aligned}
    \min_{\vx} \quad & \frac{1}{2} \vx^{\top}\mP\vx + \vq^{\top}\vx  \\
    \text{subject to} \quad & \vl \leq \mA\vx \leq \vu \text{,}
\end{aligned}    
\end{equation}
where $x \in \mathbb{R}^{N}$ is the decision variable, $\mP\in \mathbb{S}_{+}^{N}$ is the positive semi-definite quadratic cost matrix, $\vq \in \mathbb{R}^N$ is the linear cost term, $\mA \in \mathbb{R}^{M \times N}$ is a $M \times N$ matrix that describes the constraints, and $\vl$ and $\vu$ are the lower and upper bounds of constraints. Except the special cases (e.g., $\mA=0$), QP generally has no closed form solutions. As a result, QP is generally solved via some iterative methods.

\paragraph{First-order QP solver} Out of the iterative methods to solve QP, alternating direction method of multipliers (ADMM) \ch{has attracted considerable interest in recent years in different application fields, especially due to the simplicity of the iteration. (\ndref{} + I take this sentence from one of the ref. we need to properly paraphrase this.)} ADMM solves a given QP($\mP, \vq, \vl, \mA, \vu$) through the following iterative scheme. At each step $t$, It update three variables $x^{t} \in \mathbb{R}^N$ and $y^{t}, z^{t} \in \mathbb{R}^M$ as follows:
\begin{align}
    \begin{bmatrix}
        P + \sigma I & A^T \\
        A & \text{diag}(\rho)^{-1}
    \end{bmatrix}
    \begin{bmatrix}
        x^{t+1}  \\
        \nu^{t+1} 
    \end{bmatrix}
    =
    \begin{bmatrix}
        \sigma x^{t} - q\\
        z^{t} - \text{diag}(\rho)^{-1}y^{t} 
    \end{bmatrix}
    \text{,}
    \label{eq:kkt_linsys}
\end{align}
where $\sigma > 0$ is small positive constant to assure the \ch{some proper explanation}, $\rho \in \mathbb{R}^N$ is the step size parameter, and $\text{diag}(\rho) \in \mathbb{R}^{M \times M}$ is a diagonal matrix whose diagonal elements are $\rho$. By solving \cref{eq:kkt_linsys}, ADMM finds $x^{t+1}$ and $\nu^{t+1}$. After, it update $y^{t}$ and $z^{t}$ with the following equations:
\begin{align}
    \tilde{z}^{t+1} &\leftarrow{} z^{t} + \text{diag}(\rho)^{-1} (\nu^{t+1}-y^{t}) \\
    z^{t+1} &\leftarrow{} \Pi (\tilde{z}^{t}+\text{diag}(\rho)^{(-1)}y^{t}) \\
    y^{t+1} &\leftarrow{} x^{t} + \text{diag}(\rho)(\tilde{z}^{t+1} - z^{t+1}) \text{,}
\end{align}
where $\Pi$ is the projection onto the hyperbox $[\vl, \vu]$. ADMM terminates the iteration until the primal $r_{\text{primal}}^{t}=\mA x^{t}-z^{t} \in \mathbb{R}^{M}$ and dual residuals $r_{\text{dual}}^{t}=\mP x^{t}+\vq+\mA^{\top}y^{t} \in \mathbb{R}^{N}$ are sufficiently small. For instance, the termination criteria is as follows:
\begin{align}
    ||r_{\text{primal}}^{t}||_{\infty} \leq \epsilon_{\text{primal}} \text{,}
    ||r_{\text{dual}}^{t}||_{\infty} \leq \epsilon_{\text{dual}} \text{,}
\end{align}
where $\epsilon_{\text{primal}}$ and $\epsilon_{\text{dual}}$ are sufficiently small positive numbers.

\paragraph{On selection of $\rho$} As like the other numerical (iterative) optimization methods, the step-size parameter $\rho$ dominates the convergence speed of ADMM meaning that a proper choice of $\rho$ decrease the required number of iteration to find solutions. \ch{In theory, the optimal choice of $\rho$ is known. However, computing such $\rho$ is usually intractable.} Thus, various heuristics and theoretically-proven method are used to choose $\rho$ \ndref{}. \ch{Out of $\rho$ choosing mechanisms, the adaptive methods, which use the step-dependent step-size $\rho^{t}$, empirically shows relative performance advantages to the fixed step sizes.} Nonetheless, designing such adaptive rule requires tremendous efforts and also might undergoes fine tunes of rules for specific QP domains or sizes.

==> sections/method_subscript.tex <==
\label{section:method}
In this section, we present \ourmethodfull{} (\ourmethod{}) that learns to accelerate the iterative steps of ADMM. 
We first introduce the contextual MDP formulation of ADMM iterations for solving QP problems, and discuss two mechanisms that are devised to extract the spatio- and temporal-context from the ADMM iterations.


% In this section, we present First-Order Context-based Adaptation (\ourmethod{}) to learn to jointly identify and predict systems in the same family. We first introduce the training problem of \ourmethod{} and then discuss the EMA-based training method for efficiently solving the training problem.


\subsection{Contextual MDP formulation}
As we aim to develop a solver that applies to the QP problems, the learned solver is required to solve QP problems that were not seen during training. Unlike most RL applications focusing on learning a policy that solves one MDP (e.g., learning a robot manipulation policy with the fixed robot parameters), it becomes crucial that the learned solver is generalizable among QPs. To explicitly handle such effect, we model the iterative solution finding procedure of ADMM as a contextual MDP.

Assuming we have a $\text{QP}(\mP, \vq, \mA, \vl, \vu)$, where $\mP, \vq, \mA, \vl, \vu$ are the parameters of the QP problem, and $\text{ADMM}(\phi)$, where $\phi$ is the parameters of the ADMM algorithm. We then define the contextual MDP $\mathcal{M}=\big(\sX,\sU,T_\rho^c,R, \gamma)$, where $\sX=\{(x^{t}, y^{t},z^{t})\}_{t=1,2,...}$ is the set of states, $\sU=\{\rho^{t}\}_{t=1,2,...}$ is the set of actions, $T_\rho^c(x,x')=P(x^{(t+1)}=x'|x^{t}=x,\rho^{t}=\rho, c)$ is the transition function whose behaviour is contextualized  with the context $c=\{\mP, \vq, \mA, \vl, \vu, \phi\}$, $R$ is the reward function that returns 0 when  $x^{t}$ is the terminal state (i.e., the QP problem is solved) and -1 otherwise, and $\gamma \in [0,1)$ is a discount factor. As shown in the definition of $T_\rho^c$, the dynamics of MDP alters to $c$ (i.e., $T_\rho^c \neq T_\rho^{c'}$ to the given state $x$). Therefore, using the information of $c$ becomes crucial to derive the policy $\pi_\theta(x^{t})$ that minimizes the MDP steps (i.e., decreasing the ADMM steps).

One possible approach to accommodate $c$ is manually designing a feature that serves as a (minimal) sufficient statistic that separates $T_\rho^c$ from the other $T_\rho^{c'}$. However, designing such a feature can involve enormous efforts; thus, it derogates the applicability of learned solvers to the new solver classes. Instead of designing the feature, we propose to learn an context encoder that extracts the context information from the state information so that we can automate the design process. To successfully extract the context information from the states, we consider the relationship among the primal and dual variables, and QP parameters within the given state (i.e., the spatial correlation), and also their temporal correlations. To consider such spatio-temporal correlations, we propose an encoder network that is parameterized via a GNN followed with RNN \ch{Figure XX visualizes the overall network architecture.}

\subsection{Extracting spatial context information via heterogeneous graph neural network}

\paragraph{Heterogeneous graph representation of QP.} The primal $x^{t}$ and dual $y^{t}$ variables of QP are related via the QP parameters ($\mP, \vq, \mA, \vl, \vu$). As shown in \ch{Fig XX}, their relationship can be modeled as \ch{a graph} where the node represent the primal and dual variables, and the edges represents the relationship among the variables. As the roles of primal and dual variables in solving QP are distinctive, it necessitates the graph representation that reflects the different variable type information. Regarding that, we represent the relationships of the variables at $t$ th MDP steps with a directed heterogeneous graph $\gG^{t}=(\sV^{t}, \mathbb{E}^{t})$. In the following explanation, we omit the step index $t$ for notational brevity, since the graph construction is only associated with the current $t$. $\gG$ is defined as the following paragraphs.

The node set $\sV$ consist of the primal $\sV_{\text{primal}}$ and dual node set $\sV_{\text{daul}}$. The $n$ th primal and $m$ th dual nodes have node feature $(s_{\text{primal}})_n$ and $(s_{\text{dual}})_m$ defined as:
\begin{align}
(s_{\text{primal}})_n =[\underbrace{\log_{10} (r_{\text{dual}})_n, \log_{10} ||r_{\text{dual}}||_{\infty}, \mathds{1}_{({r_{\text{dual}})_n} < \eps_{\text{dual}}}}_{\text{Encoding ADMM state}}],
\end{align}
\begin{equation}
    \begin{aligned}
        (s_{\text{dual}})_m &=[\underbrace{\log_{10} (r_{\text{primal}})_m, \log_{10} ||r_{\text{primal}}||_{\infty}, \mathds{1}_{({r_{\text{primal}})_m} < \eps_{\text{primal}}}, y_m, \rho_m}_{\text{Encoding ADMM state}}, \\
        \phantom{s^{\text{primal}}_m} & \underbrace{\min(z_m-l_m,u_m-z_m),
        \mathds{1}_{\text{equality}}, \mathds{1}_{\text{inequality}}}_{\text{Encoding QP structure}}] \text{,}
    \end{aligned}        
\end{equation} $(r_{\text{primal}})_n$ and $(r_{\text{dual}})_m$ denotes the $n$ th and $m$ th element of primal and dual residual, respectively, \ch{$\mathds{1}_{(r_{\text{primal}})_m < \eps_{\text{primal}}}$ and $\mathds{1}_{(r_{\text{dual}})_m < \eps_{\text{dual}}}$ are the indicators whether the $n$ th primal and $m$ th dual residual converge, respectively}, $\mathds{1}_{\text{equality}}$ and $\mathds{1}_{\text{inequality}}$ are the indicators whether $m$ th constraint is equality and inequality, respectively. \ch{Explain about the ADMM state and QP structure}.

The edge set $\mathbb{E}$ consist of the following edge sets:
\begin{itemize}[leftmargin=0.5cm]
    \item The primal-to-primal edge set $\mathbb{E}^{\text{p2p}}$ is defined as $\{e^{\text{p2p}}_{ij}| \mP_{ij} \neq 0 \, \forall (i,j) \in [\![1,N]\!] \times [\![1,N]\!] \}$ where $[\![1,N]\!]=\{1,2,..,N\}$. i.e., the edge from the $i$ th primal node to $j$ th primal node exists when the corresponding $\mQ$
    % smalll q 어떻게 적죠...
    is not zero. The edge $e^{\text{p2p}}_{ij}$ has the feature $s_{ij}^{\text{p2p}}$ as $[\mP_{ij},q_i]$.
    \item The primal-to-dual edge set $\mathbb{E}^{\text{p2d}}$ is defined as $\{e_{ij}| \mA_{ji} \neq 0 \, \forall (i,j) \in [\![1,N]\!] \times [\![1,M]\!] \}$. The edge $e^{\text{p2d}}_{ij}$ has the feature $s_{ij}^{\text{p2d}}$ as $[A_{ji}]$. 
    \item The dual-to-primal edge set $\mathbb{E}^{\text{d2p}}$ is defined as $\{e_{ij}| \mA_{ij} \neq 0 \, \forall (i,j) \in [\![1,M]\!] \times [\![1,N]\!] \}$. The edge $e^{\text{d2p}}_{ij}$ has the feature $s_{ij}^{\text{d2p}}$ as $[A_{ij}]$. 
\end{itemize}

\paragraph{Graph preprocessing for unique QP representation.} QP problems has the same optimal decision variables to the affine transforms to objective function and constraints. However, the transformed QP is represented as a different graph to the graph representation of the original QP problem. To take account the effect of such transformations, we scale the QP problems so that they become invariant to the affine transformations. \ch{The details of the preprocessing steps are given in Appendix XX.}

\paragraph{Comparison to \model{RLQP} representation. } \ch{-----------}

\paragraph{Grpah embedding with Hetero GNN.} The heterogeneous graph $\gG$ models the various type of information among the primal and dual variables. To take account such type information for the node and edge embedding, we use hetero graph attention (HGA), \ch{a variant of type-aware graph attention \citep{park2021schedulenet}, to embed $\gG$.} the hetero graph attention (HGA). HGA employs the separate node and edge encoders for each node and edge type. It computes the edge embedding with the edge encoders per edge types. After, it applies the attention mechanism to compute the weight factors for each type of edges. With the computed weight and edge embedding, it computes the aggregated edge embedding by performing the weighted summation per types. Then it sums the different-typed aggregated edge embedding to form the type-independent edge embedding. Lastly, HGA updates the node embedding by using the type-independent edge embedding as an input of node encoders. Due to the page limit, we provide the details of HGA in Appendix.


% is composed of 'edge update,' 'edge aggregation,' 'node update,' and 'hetero node aggregation' to extract informative context by considering each edge type and compute the updated node, edge embeddings as follows:


% \ch{
% \begin{itemize}[leftmargin=0.5cm]
%     \item The node set $\sV=\sV_{\text{primal}} \cup \sV_{\text{dual}}$, where $\sV_{\text{primal}}$ and $\sV_{\text{dual}}$ are the set of primal and dual variables, respectively. We define the primal node features of node $v^j_{\text{primal}}$, $s^{j}_{\text{primal}}$ and the dual node feature s$v^i_{\text{dual}}$, $s^{i}_{\text{primal}}$ as: \\$s^{j}_{\text{primal}} =
%     \begin{bmatrix}
%     \log_{10}{\xi_{dual}^j} \\  
%     \xi_{dual}^j < \xi_{dual}^j \text{'s tolerance}\\
%     \log_{10}{||\xi_{dual}||_{\infty}} \\  
%     \end{bmatrix}
%     $, 
%     $s^{i}_{\text{dual}} =
%     \begin{bmatrix}
%     \log_{10}{\xi_{primal}^i} \\  
%     \xi_{primal}^i < \epsilon\\ % \xi_{primal}^i \text{'s tolerance}\\
%     \log_{10}{||\xi_{primal}||_{\infty}} \\
%     y \\
%     \min(z_i - l_i, u_i - z_i)\\
%     u_i \\
%     \text{inequality}\\
%     \text{equality}\\
%     \end{bmatrix}
%     $ 
%     \item The edge set $\mathbb{E}=\mathbb{E}_{\text{p2p}} \cup \mathbb{E}_{\text{p2d}} \cup \mathbb{E}_{\text{d2p}}$, where $\mathbb{E}_{\text{p2p}}$ is the set of edges between primal and primal variables to express the objective function's parameter $\mP, \vq$, and $ \mathbb{E}_{\text{p2d}}, \mathbb{E}_{\text{d2p}}$ are the set of edges between primal and dual variables, and dual and primal variables to express constraint's parameter $\mA$, respectively.
%     We define the edge features of $e_{ij}$ as: \\
%     \[
%       e_{ij} = \left.
%       \begin{cases}
%         [P_{ij}, q_{i}], & \text{for } i=j, e_{ij} \in \mathbb{E}_{\text{p2p}} \\
%         [P_{ij}, 0], & \text{for } i\neq j, e_{ij} \in \mathbb{E}_{\text{p2p}}\\
%         [A_{ij}], & \text{for } e_{ij} \in \mathbb{E}_{\text{d2p}} \\
%         [A_{ji}], & \text{for } e_{ij} \in \mathbb{E}_{\text{p2d}} \\
%       \end{cases}
%       \right\}
%     \]
%     % e^{d2p}_{ij} = \begin{bmatrix}A_{ij}   \end{bmatrix},
%     % e^{p2d}_{ij} = \begin{bmatrix} A_{ji} \end{bmatrix}
% \end{itemize}
% }

% \ch{[\textbf{Mention the state pre-processing steps.}] There is a problem with taking the values of QP parameters $\mP, \vq, \mA, \vl, \vu$ as they are. Because a single objective function or constraint can be expressed in various ways. For example, $x_1 + x_2 \leq 2$ and $2x_1 + 2x_2 \leq 4$ are the same constraints, but they have different coefficients. Therefore, data scaling was performed to solve this problem. The detail scaling algorithms for constraint and objective functions are provided in \ref{alg:constraint_scaling}, \ref{alg:objective_scaling} in Appendix \ref{Matrix-Scaling}, respectively.}

% \ch{The heterogeneous graph $\gG$ models the various type of information among the primal and dual variables. To take account such type information for the node and edge embedding, we propose to utilize the following hetero graph attention (HGA). HGA is composed of 'edge update,' 'edge aggregation,' 'node update,' and 'hetero node aggregation' to extract informative context by considering each edge type and compute the updated node, edge embeddings as follows:}
% Assume performing HGA with edge type $k$ that connects node type $k_s$ and $k_d$. And the index of source node and destination node is $i$, $j$ respectively. Therefore Given the source node embedding is $h^{k_s}_i$, the destination node embedding is $h^{k_d}_j$, and the edge node embedding is $h^{k}_{ij}$.

% \textbf{Edge update} Given the node embedding $h_i, h_j$ and the edge embedding $h_{ij}$ with edge type $k$, HGA computes the type-specific edge embedding ${h'_{ij}}$, and the attention logit $z_{ij}$ as:
% \begin{align}
%     h'_{ij} = \text{HGA}^{k}_{E}([h_i, h_j, h_{ij}]) \\
%     z_{ij} = \text{HGA}^{k}_{A}([h_i, h_j, h_{ij}]) 
% \end{align}
% where $\text{HGA}^{k}_{E}$ and $\text{HGA}^{k}_{A}$ are the hetero edge update function and the hetero attention function for edge type $k$, respectively. Both functions are composed of Multilayer Perceptron (MLP). %(The dimension of the first layer and the dimension of the last layer may be different depending on the edge type).  Relation between variables and relation between constraints and variables are fundamentally different. Therefore, if it is a different edge type, edge embedding and attention logit were made to be completed through different functions for extracting meaningful embeddings.
% 장점 적어야함

% \textbf{Edge aggregation}  Each edge has a different part of being expressed within QP. Therefore, to consider other edge types' characteristics, the aggregation of message $h'_{ij}$ proceeds for each edge type. \\
% First, HGA computes attention $\alpha_{ij}$ corresponding to the $h'_{ij}$ as:
% \begin{align}
%     \alpha_{ij} = \frac{\exp(z_{ij})}{\sum_{i\in N_k(j)} \exp(z_{ij})}
% \end{align}

% where $N_{k}(j)=\{v_i |\text{type of }e_{ij} : k, v_j \in N(i)\  \forall i\}$ is the set of all neighborhood of $v_j$, which type of edge from the element of the set to $v_j$ is $k$. \\
% Second, HGA aggregates messages and produces the type $k$ message $m^k_j$ for node $v_{j}$.
% \begin{align}
%     m^{k}_{j} = \sum_{i\in N_k(j)} \alpha_{ij} h'_{ij}
% \end{align}

% 다른 이름 필요해 보임....
% \textbf{Edge type-aware node update} The aggregated message with edge type $k$, $m^k_j$ is used to computed, updated node embedding with edge type $k$, ${\mathfrak{h}^{k}_j}'$ as: 
% \begin{align}
%     {\mathfrak{h}^{k}_j} = \text{HGA}^{k}_V ([h_j, m^k_j])
% \end{align}
% where $\text{HGA}^{k}_{V}$ is the hetero node update function, which is composed of MLP.

% The above three steps (Edge update, Edge aggregation, Edge type-aware node update) are performed separately on each edge type to preserve the characteristics of the edge type and extract meaningful embedding.
% %The detailed structure of $\text{HGA}^{k}_E$, $\text{HGA}^{k}_A$, and $\text{HGA}^{k}_V$ are provided in Appendix. %!!!appendix section 필요!!!

% \textbf{Node aggregation} HGA aggregated updated hetero node feature ${\mathfrak{h}^{k}_j}$ to produce updated node embedding $h_j'$ as following procedures.\\
% First, HGA computes attention logit $d^k_j$ corresponding to the ${\mathfrak{h}^{k}_j}'$ as:
% \begin{align}
%     d^k_j = \text{HGA}_N({\mathfrak{h}^{k}_j}')
% \end{align}
% where $\text{HGA}_{N}$ is the hetero node update function, which is composed of MLP.\\
% Second, HGA computes attention $\beta^k_j$ with $d^k_j$ and softmax function as:
% \begin{align}
%     \beta^k_j = \frac{\exp(d^k_j)}{\sum_{k\in E_{dst}(j)} \exp(d^k_j)}
% \end{align}
% where $E_{dst}(j)$ is the set of edge types which has a destination node at $j$.\\
% Finally, HGA aggregates the per-type updated messages to compute updated node feature $h'_j$ for $v_j$ as:
% \begin{align}
%     h'_j = \sum_{k\in E_{dst}(j)} \beta^k_j {\mathfrak{h}^{k}_j}'
% \end{align}



\subsection{Extracting temporal context via RNN}
In the previous section, we discuss how to extract context by considering the spatial correlation among the variables within the MDP step. We then discuss how to extract the temporal correlations. At the $t^{\text{th}}$ MDP step, we consider $l$ historical state observations to extract the temporal context. Specifically, we first apply HGA to $\gG^{t-l}, ..., \gG^{t-1}$ and then apply GRU \ndref{} as follows:
\begin{align}
    \sG^{t-l+\delta} &= \text{HGA}(\gG^{t-l+\delta}) \qquad &\text{for } \delta &= 0, 1, 2, \cdots , l-1 \\
    \gH^{t-l+\delta} &= \text{GRU} ({\sV^{t-l+\delta}}, \gH^{t-l+\delta-1}) \qquad &\text{for } \delta &= 1, 2, \cdots , l-1 % 
\end{align} 
where $\sG^{t-l+\delta}$ is updated graph at $t-l+\delta$ step, $\sV^{t-l+\delta}$ is the set of update node of $\sG^{t-l+\delta}$, $\gH^{t-l+\delta}$ is the set of hidden embedding at $t-l+\delta$. We define the node-wise context $\gC^{t}$ at time $t$ as the last hidden embedding $\gH^{t-1}$.

\paragraph{Policy and value network design and training} We parameterize the policy $\pi_\theta(\gG^{t}, \gC^{t})$ via the HGA followed by MLP. Since action $\rho^{t}$ is not defined at $t$, we exclude $\rho^{t}$ from the node features of $\gG^{t}$ instead node-wisely concatenate $\gC^{t}$ to the node features. For the action-value network $Q_\theta(\gG^{t}, \rho^{t}, \gC^{t})$, we use $\gG^{t}$ and $\gC^{t}$ as the input. $Q_\theta(\gG^{t}, \rho^{t}, \gC^{t})$ has the same network architecture of $\pi_\theta(\gG^{t}, \gC^{t})$. We train $\pi_\theta(\gG^{t}, \gC^{t})$ and $Q_\theta(\gG^{t}, \rho^{t}, \gC^{t})$ on the QP problems of size 10$\sim$15 (i.e., 10$\sim$15 primal variables) with DDPG \ndref{} algorithm. Please refer the \ch{Appendix ??} for the details of network architecture and training.


% Contextual-RLQP uses history to overcome the weaknesses of a single state's markovian, improve understanding of dynamic systems, and extract context from contextual learning. In other words, it allows the critic and actor networks to estimate the correct future reward and search for the optimal policy. \\
% In the algorithm, the informative context was inferred from the history using the GRU of the RNN family. We used history with a fixed length of $l$ to facilitate learning through a batch. At the same time, history includes the action of the past timestep for providing more information. Therefore, the definition of history with length $l$ at timestep $t$, $\mathcal{H}^{t}$ is as follows.
% \begin{align}
%     \mathcal{H}^{t} \coloneqq [[G^{t-l}, a^{t-l}],[G^{t-l+1}, a^{t-l+1}],...,[G^{t-1}, a^{t-1}]]
% \end{align}
% where $G^{t}$ is graph representation of QP at timestep $t$. The meaning of $[G^{t}, a^{t}]$ is that $G^{t}$ and $a^{t}$ are concatenated. The $a^{t}$ was concatenated on the corresponding dual node features of $G^{t}$.

==> tables/ablation_model.tex <==
\begin{table}[]
    \caption{\textbf{Ablation study models}}
    \centering
    \resizebox{0.4\textwidth}{!}{
    \begin{tabular}{cccc}
    \toprule
    & Heterograph repr. & HGA & GRU \\
    \cmidrule(lr){1-1}\cmidrule(lr){2-2}\cmidrule(lr){3-3}\cmidrule(lr){4-4}
    \model{RLQP} & $\textcolor{red}{\xmark}$ & $\textcolor{red}{\xmark}$ & $\textcolor{red}{\xmark}$ \\
    \cmidrule(lr){1-1}\cmidrule(lr){2-2}\cmidrule(lr){3-3}\cmidrule(lr){4-4}
    \model{HGA} & $\textcolor{codegreen}{\cmark}$ & 
    $\textcolor{codegreen}{\cmark}$ &
    $\textcolor{red}{\xmark}$ \\
    \cmidrule(lr){1-1}\cmidrule(lr){2-2}\cmidrule(lr){3-3}\cmidrule(lr){4-4}
    \model{\ourmethod{}}&
    $\textcolor{codegreen}{\cmark}$ & $\textcolor{codegreen}{\cmark}$ & $\textcolor{codegreen}{\cmark}$ \\
    \bottomrule
    \end{tabular}
    }
    \label{table:ablation_models}
\end{table}

% \begin{table}[]
%     \caption{\textbf{Ablation study models (small size random QP).} Best in \textbf{bold}. We measure the average and standard deviation of ADMM iterations for each QP benchmark. All QP problems are generated to have $10 \leq N \leq 15$.}
%     \centering
%     \resizebox{0.65\textwidth}{!}{
%     \begin{tabular}{ccccc}
%     \toprule
%     & Heterograph rep. & HGA & GRU & ADMM iterations\\
%     \cmidrule(lr){1-1}\cmidrule(lr){2-2}\cmidrule(lr){3-3}\cmidrule(lr){4-4}\cmidrule(lr){5-5}
%     % \makecell{\model{HGA+GRU} \\ (\model{\ourmethod{}})}&
%     \model{\ourmethod{}}&
%     $\textcolor{codegreen}{\cmark}$ & $\textcolor{codegreen}{\cmark}$ & $\textcolor{codegreen}{\cmark}$ &
%     24.24 $\pm$ 4.66 \\
%     \cmidrule(lr){1-1}\cmidrule(lr){2-2}\cmidrule(lr){3-3}\cmidrule(lr){4-4}\cmidrule(lr){5-5}
%     \model{HGA} & $\textcolor{codegreen}{\cmark}$ & 
%     $\textcolor{codegreen}{\cmark}$ &
%     $\textcolor{red}{\xmark}$ &
%     \textbf{22.86} $\pm$ 3.26 \\
%     \cmidrule(lr){1-1}\cmidrule(lr){2-2}\cmidrule(lr){3-3}\cmidrule(lr){4-4}\cmidrule(lr){5-5}
%     % \model{GRU} & $\textcolor{red}{\xmark}$ & 
%     % $\textcolor{red}{\xmark}$ &
%     % $\textcolor{codegreen}{\cmark}$ & 
%     % 83.56 $\pm$ 29.16 \\
%     \cmidrule(lr){1-1}\cmidrule(lr){2-2}\cmidrule(lr){3-3}\cmidrule(lr){4-4}\cmidrule(lr){5-5}
%     \model{RLQP} & $\textcolor{red}{\xmark}$ & $\textcolor{red}{\xmark}$ & $\textcolor{red}{\xmark}$ &
%     67.90 $\pm$ 38.56 \\
%     \bottomrule
%     \end{tabular}
%     }
%     \label{table:ablation_models}
% \end{table}

==> tables/ablation_model_large_qp.tex <==
\begin{table}[t]
    \centering
    \caption{\textbf{Ablation study results (larger size random QP).} Best in \textbf{bold}. We measure the average and standard deviation of ADMM iterations.}
    \resizebox{1.0\textwidth}{!}{
    \begin{tabular}{cccccccccc}
    \toprule
    & \multicolumn{8}{c}{Problem size ($N$)} \\
    % Second row
    &
    100 $\sim$ 200 & 
    200 $\sim$ 300 & 
    300 $\sim$ 400 & 
    400 $\sim$ 500 & 
    500 $\sim$ 600 & 
    600 $\sim$ 700 & 
    700 $\sim$ 800 & 
    800 $\sim$ 900 & 
    900 $\sim$ 1000\\
    \cmidrule(lr){1-1}\cmidrule(lr){2-2}\cmidrule(lr){3-3}\cmidrule(lr){4-4}\cmidrule(lr){5-5}\cmidrule(lr){6-6}\cmidrule(lr){7-7}\cmidrule(lr){8-8}\cmidrule(lr){9-9}\cmidrule(lr){10-10}
    \model{RLQP} &
    \makecell{81.81 \\ $\pm$ 13.45} &
    \makecell{103.41 \\ $\pm$ 12.66} &
    \makecell{133.102 \\ $\pm$ 10.12} &
    \makecell{155.55 \\ $\pm$ 10.10} &
    \makecell{168.96 \\ $\pm$ 9.82} &
    \makecell{184.60 \\ $\pm$ 9.64} &
    \makecell{198.50 \\ $\pm$ 9.41} &
    \makecell{212.10 \\ $\pm$ 9.14} &
    \makecell{223.30 \\ $\pm$ 7.92} \\
    % Third row
    \cmidrule(lr){1-1}\cmidrule(lr){2-2}\cmidrule(lr){3-3}\cmidrule(lr){4-4}\cmidrule(lr){5-5}\cmidrule(lr){6-6}\cmidrule(lr){7-7}\cmidrule(lr){8-8}\cmidrule(lr){9-9}\cmidrule(lr){10-10}
    \model{HGA} &
    \makecell{\textbf{38.61} \\ $\pm$ 4.47} &
    \makecell{\textbf{47.06} \\ $\pm$ 3.53} &
    \makecell{\textbf{51.51} \\ $\pm$ 3.05} &
    \makecell{\textbf{55.59} \\ $\pm$ 2.47} &
    \makecell{\textbf{58.37} \\ $\pm$ 2.27} &
    \makecell{61.08 \\ $\pm$ 2.59} &
    \makecell{64.46 \\ $\pm$ 2.55} &
    \makecell{65.94 \\ $\pm$ 2.18} &
    \makecell{68.94 \\ $\pm$ 2.76} \\
    \cmidrule(lr){1-1}\cmidrule(lr){2-2}\cmidrule(lr){3-3}\cmidrule(lr){4-4}\cmidrule(lr){5-5}\cmidrule(lr){6-6}\cmidrule(lr){7-7}\cmidrule(lr){8-8}\cmidrule(lr){9-9}\cmidrule(lr){10-10}
    \model{\ourmethod{}} &
    \makecell{41.92 \\ $\pm$ 5.69} &
    \makecell{50.35 \\ $\pm$ 4.08} &
    \makecell{54.41 \\ $\pm$ 3.81} &
    \makecell{57.00 \\ $\pm$ 3.15} &
    \makecell{59.43 \\ $\pm$ 3.95} &
    \makecell{\textbf{59.88} \\ $\pm$ 3.10} &
    \makecell{\textbf{62.92} \\ $\pm$ 3.31} &
    \makecell{\textbf{65.92} \\ $\pm$ 4.00} &
    \makecell{\textbf{67.00} \\ $\pm$ 3.27} \\
    \bottomrule
    \end{tabular}
    }
    \label{tab:ablation_model_larger_qp}
\end{table}
